Lesion Localization in OCT by Semi-Supervised Object Detection

Over 300 million people worldwide are affected by various retinal diseases. By noninvasive Optical Coherence Tomography (OCT) scans, a number of abnormal structural changes in the retina, namely retinal lesions, can be identified. Automated lesion localization in OCT is thus important for detecting retinal diseases at their early stage. To conquer the lack of manual annotation for deep supervised learning, this paper presents a first study on utilizing semi-supervised object detection (SSOD) for lesion localization in OCT images. To that end, we develop a taxonomy to provide a unified and structured viewpoint of the current SSOD methods, and consequently identify key modules in these methods. To evaluate the influence of these modules in the new task, we build OCT-SS, a new dataset consisting of over 1k expert-labeled OCT B-scan images and over 13k unlabeled B-scans. Extensive experiments on OCT-SS identify Unbiased Teacher (UnT) as the best current SSOD method for lesion localization. Moreover, we improve over this strong baseline, with mAP increased from 49.34 to 50.86.

==> backup.tex <==
\begin{itemize}
  \item [1] 
  {\bfseries Score filter} Use box candidates meet $f(b)>\theta$ as the pseudo label, where $\theta $ is a given threshold and $f(\cdot)$ is the foreground score of the box candidate. Note that the foreground score is defined as the maximum probability of all non-background categories.
%   \item [2]
%   {\bfseries N.A.} Don't generate the pseudo label for box regression losses calculation. 
  \item [2]
  {\bfseries Double filter} Use box candidates meet $f(b)>\theta_{2} \And r(b)>\delta $ as the pseudo label for regression losses, where $\theta_{2}$ and $\delta$ are given thresholds and $r(\cdot)$ is box regression variance of the box candidate.
\end{itemize}

Specifically, we get the refined box $\hat{b}$ by feeding the jittered box around given box candidate $b$ into the teacher model, which is formulated as follows:$\hat{b}=refine(jitter(b))$. Repeat the above procedure several times , we get a set of $N_{jitter}$ refined jittered boxes $\{b_{i}\}$, and the box regression variance can be computed as:
\begin{equation}
r(b)=\frac{1}{4}\sum_{k=1}^{4}\frac{\sigma_{k}}{0.5(h(b)+w(b))}
\label{reg}
\end{equation}
where $\sigma_{k}$ is the standard derivation of the k-th coordinate of the refined jittered boxes set $\{ b_{i}\}$, $h(b)$ and $w(b)$ represent the height and width of box candidate $b$, respectively. 

As for the pseudo labels generation strategy for classification loss calculation, they all use the foreground score threshold strategy.


\subsection{The overview framework}
There are two models with the same structure, called student and teacher in the framework. As shown in Figure \ref{fig2}, the training steps are summarized as follows:

\begin{itemize}
  \item [1]
  {\bfseries Teacher initialization/update.} 
  
  \item [2] 
  {\bfseries Pseudo label generation.} Given an unlabeled image $x_u$, the teacher model $p_{t}$ is performed to generate box candidates on unlabeled data applied weak augmentations $a(\cdot)$. By using some strategies $PLG(\cdot)$, we get $c_{u}$ and $b_{u}$, which are pseudo label for $\ell_{cls}$ and $\ell_{reg}$ computation.
    \begin{equation}
     \{c_{u},b_{u}\}=PLG(p_{t}( c,b\mid a(x_{u}))) \label{pre}
    \end{equation}
  \item [3]
  {\bfseries Student training.} The student model $p_{s}$ uses unlabeled data applied strong augmentations $A(\cdot) $ with pseudo label as the ground-truth and labeled data with the ground-truth for training by jointly minimizing supervised loss and unsupervised loss, denoted as $\ell_{s}$ and $\ell_{u}$. Go back to step 1.
    \begin{equation}
    \ell=\ell_{s}+\lambda_{u}\ell_{u}  \label{loss_t}
    \end{equation}
\end{itemize}


$\lambda_{u}$ is to balance supervised loss $\ell_{s}$ and unsupervised loss $\ell_{u}$ in function \ref{loss_t}. The supervised loss $\ell_{s}$ and unsupervised loss $\ell_{s}$ consists of classification loss $\ell_{cls}$ and regression loss $\ell_{reg}$, which can be written as: 

\begin{equation}
\begin{split}
\ell_{s}=\frac{1}{N_{l}}\sum \ell_{cls}(p_{s}(c \mid A(x_{l}), a(x_{l})),c_{l})
\\+\lambda _{r}\ell_{reg}(p_{s}(b\mid A(x_{l}), a(x_{l})),b_{l})
\label{suploss}
\end{split}
\end{equation}

\begin{equation}
% \begin{split}
\ell_{u}=\frac{1}{N_{u}}\sum \ell_{cls}(p_{t}(c \mid A(x_{u})),c_{u})
+\lambda _{r}\ell_{reg}(p_{t}(b \mid A(x_{u})),b_{u})
\label{unsuploss}
% \end{split}
\end{equation}

In the above equation, $\lambda _{r}$ is $N_{l}$ and $N_{u}$ are batch size of labeled and unlabeled B-scans respectively. 


\begin{itemize}
\item {\verb|Faster RCNN|}: 
A standard Faster R-CNN with FPN and ResNet-50 backbone. We include this baseline as the supervised baseline for a more comprehensive evaluation. The data augmentations are flip and color transformation.
\item {\verb|Unbiased Teacher|}: 
In our implementation, we follow most of the experimental parameter settings of Unbiased Teacher\cite{liu2021unbiased}. For large-scale Cutout that may completely cut a lesion, we reduce the scale and ratio parameters of cutup in strong data augmentations.  
\item {\verb|Soft Teacher|}: 
In our implementation, we follow most of the experimental parameter settings of Soft Teacher\cite{xu2021end}. For large-scale Cutout that may completely cut a lesion, we reduce the scale and ratio parameters of cutup in strong data augmentations.  
\end{itemize}

